AMUSE: Adaptive Multi-Segment Encoding for Dataset Watermarking

Curating high quality datasets that play a key role in the emergence of new AI applications requires considerable time, money, and computational resources. So, effective ownership protection of datasets is becoming critical. Recently, to protect the ownership of an image dataset, imperceptible watermarking techniques are used to store ownership information (i.e., watermark) into the individual image samples. Embedding the entire watermark into all samples leads to significant redundancy in the embedded information which damages the watermarked dataset quality and extraction accuracy. In this paper, a multi-segment encoding-decoding method for dataset watermarking (called AMUSE) is proposed to adaptively map the original watermark into a set of shorter sub-messages and vice versa. Our message encoder is an adaptive method that adjusts the length of the sub-messages according to the protection requirements for the target dataset. Existing image watermarking methods are then employed to embed the sub-messages into the original images in the dataset and also to extract them from the watermarked images. Our decoder is then used to reconstruct the original message from the extracted sub-messages. The proposed encoder and decoder are plug-and-play modules that can easily be added to any watermarking method. To this end, extensive experiments are preformed with multiple watermarking solutions which show that applying AMUSE improves the overall message extraction accuracy upto 28% for the same given dataset quality. Furthermore, the image dataset quality is enhanced by a PSNR of $\approx$2 dB on average, while improving the extraction accuracy for one of the tested image watermarking methods.

==> notation.tex <==
\subsection{Notation}
\begin{table}[th]
\caption{Notation of the paper}
\begin{tabularx}{0.5\textwidth}{p{0.03\textwidth}X}
  $\mathbf{X}$ & The original dataset  \\
  $\mathbf{x_i}$ & $i$-th sample in $\mathbf{X}$ \\
  $n$ & The number of samples in the original dataset \\
  $\mathbf{\tilde{X}}$ &  Watermarked dataset  \\
  $\mathbf{\tilde{x}_i}$ & $i$-th sample in $\mathbf{\tilde{X}}$ \\
  
  $\mathbf{\tilde{X}_s}$ &  A subset of the Watermarked dataset  \\
  
  $W$ & Watermark embedding  \\
  $\Psi$ & The watermark extraction \\
  $e_d(.)$ & The function to obtain the dataset distortion \\ 
  $e_w(.)$ & The function to obtain the message distortion \\ 
  $E$ & The encoder \\
  $D$ & The decoder \\ 
  $M$ & the original message   \\
  $M^j$ & $j$-th bit in $M$ \\
  $L$ & the length of the original message   \\
  
  $\overbar{M}$ & set of sub-messages \\ 
  $M_i$ & $i$-th embedded submessage \\
  $l$ & the length of $M_i$ \\  
  
  $\overbar{M}'$ & set of extracted submessages \\
  $M_i^{'}$ & the $i$-th extracted message \\
  $M'$ & the reconstructed message  \\
  $M'^j$ & $j$-th bit in $M'$ \\
  
  $N$ & The number of chunks \\
  $K$ & The number of excluded chunks in the submessage \\
  $C$ & The number of possible chunks combinations \\
  $p$ & The number of padding bits \\
  

  
  %$\tau$ & \textcolor{red}{Need to complete the table}
  
\end{tabularx}
\end{table}

